Extreme Acceleration of Graph Neural Network-based Prediction Models for Quantum Chemistry

Molecular property calculations are the bedrock of chemical physics. High-fidelity \textit{ab initio} modeling techniques for computing the molecular properties can be prohibitively expensive, and motivate the development of machine-learning models that make the same predictions more efficiently. Training graph neural networks over large molecular databases introduces unique computational challenges such as the need to process millions of small graphs with variable size and support communication patterns that are distinct from learning over large graphs such as social networks. This paper demonstrates a novel hardware-software co-design approach to scale up the training of graph neural networks for molecular property prediction. We introduce an algorithm to coalesce the batches of molecular graphs into fixed size packs to eliminate redundant computation and memory associated with alternative padding techniques and improve throughput via minimizing communication. We demonstrate the effectiveness of our co-design approach by providing an implementation of a well-established molecular property prediction model on the Graphcore Intelligence Processing Units (IPU). We evaluate the training performance on multiple molecular graph databases with varying degrees of graph counts, sizes and sparsity. We demonstrate that such a co-design approach can reduce the training time of such molecular property prediction models from days to less than two hours, opening new possibilities for AI-driven scientific discovery.

==> TODO_MLSys <==
Would it make sense to add packing efficiency plots for water clusters too in the draft that you guys have been discussing earlier? Also should we report/record how long it takes for LPFHP to compute the packing in each case (to report the pre-processing time for packing before starting the training)? Another thing I was wondering is whether it would be possible to report results (packing efficiency, total execution time, packing calculation time)  with any other alternative heuristics/strategies that are available and perhaps a justification for using them if any (for example, efficiency may be ~70% instead of ~98%  with an alternative technique but computing the packing may be super fast)? 

--> 

2. 500k 2-IPU run missing (for strong scaling)

3. In addition to absolute time per epoch report average execution time, speedup.

4. Include Throughput (graphs/s) plots ? -> What does throughput mean in this context?

5. Revisit whether to include "Histogram of node degree in HydroNet dataset with cutoff=6" plot

6. Include profiler output and discussion about improving the tail latency ? excerpt from slack "The (lack) of strong scaling with number of replicas was bothering me so I spent a little time today investigating and found another optimisation to apply to how the gradients are merged between replicas.  This can be seen in the “tail” of the profile on the left  The default is to appears to process one grad at a time (possibly this is the safer option for models that are close to the memory limit). I enabled a pass that effectively fuses these reductions together and the result is the profile on the right.  Running a new round of experiments to see if the difference can be observed in the epoch times." 

Link: https://torchgeometricco.slack.com/archives/C0437R43BB6/p1665605539900369

7. Revisit strong scaling ? "I’ve discussed these experiments with some of the research team and they suggested that a strong scaling study would need to maintain the same global batch size as the number of replicas is varied. In this case we would need to adjust the gradient accumulation factor accordingly to maintain the same number of examples being processed in a single overall step"

8. Overlapped I/O discussion/profiler op? "got overlapped IO working now:
left vanilla run with 8 gradient accumulation steps
enable prefetch depth of 8 + using 128 io tiles"

9. Discussion about computing interaction graph on the device instead of the host. Excerpt from slack: "a new customisable interaction_graph  method for the PyG implementation of SchNet.  The method I’ve implemented on the IPU calculates the all-to-all pairwise distance matrix, applies some masking and then uses topk to select the k-nearest neighbors for the batched graphs. "



10. "For figure 4, would it be possible to turn off the curve smoothing in the histogram? It would be more appropriate to have bars instead of curves, because for the intermediate numbers in the dips, the respective values are actually zero to the best of my knowledge."

11. Bring back "“\cite{tuple}” to reference the tuple packing paper"

12. what is difficult is comparing throughput between the datasets (e.g. QM9 is much smaller).
One solution would be to report # nodes / sec

